Video Prediction Models as Rewards for Reinforcement Learning

Specifying reward signals that allow agents to learn complex behaviors is a long-standing challenge in reinforcement learning. A promising approach is to extract preferences for behaviors from unlabeled videos, which are widely available on the internet. We present Video Prediction Rewards (VIPER), an algorithm that leverages pretrained video prediction models as action-free reward signals for reinforcement learning. Specifically, we first train an autoregressive transformer on expert videos and then use the video prediction likelihoods as reward signals for a reinforcement learning agent. VIPER enables expert-level control without programmatic task rewards across a wide range of DMC, Atari, and RLBench tasks. Moreover, generalization of the video prediction model allows us to derive rewards for an out-of-distribution environment where no expert data is available, enabling cross-embodiment generalization for tabletop manipulation. We see our work as starting point for scalable reward specification from unlabeled videos that will benefit from the rapid advances in generative modeling. Source code and datasets are available on the project website: https://escontrela.me/viper

==> figs/results_corrected/figure.tex <==


\begin{figure}[ht]
    \includegraphics[width=\textwidth]{figs/results/results_agg.pdf}
    \caption{Updated \cref{fig:results}, with correction: error bars are computed across seeds, whereas before they were mistakenly computed across tasks. Aggregate results across 15 DMC tasks, 7 Atari games, and 6 RLBench tasks. DMC results are provided for DrQ and DreamerV3 (Dv3) RL agents. Atari and RLBench results are reported for DreamerV3. Atari scores are computed using Human-Normalized Mean. }
    \label{fig:results_corrected}    
\end{figure}
